CASP-DM: Context Aware Standard Process for Data Mining

We propose an extension of the Cross Industry Standard Process for Data Mining (CRISPDM) which addresses specific challenges of machine learning and data mining for context and model reuse handling. This new general context-aware process model is mapped with CRISP-DM reference model proposing some new or enhanced outputs.

==> 2-CaspDM.tex <==
\section{CASP-DM: Phases}

\begin{figure}[htbp]
	\centering
		\includegraphics[width=0.7\textwidth]{CASPDMLIFE.pdf}
	\caption{CASP-DM Life Cycle}
	\label{fig:CASPDMLIFE}
\end{figure}


\subsection{Business Understanding}

\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.00\textwidth]{1-BusinessUnderstanding.pdf}
	\caption{Phase 1. Business understanding: tasks and activities for context-awareness}
	\label{fig:BusinessUnderstanding}
\end{figure}


\subsection{Data Understanding}

\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.00\textwidth]{2-DataUnderstanding.pdf}
	\caption{Phase 2. Data Understanding: tasks and activities for context-awareness}
	\label{fig:DataUnderstanding}
\end{figure}


\subsection{Data Preparation}

\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.00\textwidth]{3-DataPreparation.pdf}
	\caption{Phase 3. Data Preparation: tasks and activities for context-awareness}
	\label{fig:DataPreparation}
\end{figure}


\subsection{Modeling}

\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.00\textwidth]{4-Modeling.pdf}
	\caption{Phase 4. Modelling: tasks and activities for context-awareness}
	\label{fig:Modeling}
\end{figure}



\subsection{Evaluation}

\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.00\textwidth]{5-Evaluation.pdf}
	\caption{Phase 5. Evaluation: tasks and activities for context-awareness}
	\label{fig:Evaluation}
\end{figure}


\subsection{Deployment}

\begin{figure}[htbp]
	\centering
		\includegraphics[width=1.00\textwidth]{6-Deployment.pdf}
	\caption{Phase 6. Deployment: tasks and activities for reframing.}
	\label{fig:Deployment}
\end{figure}


\subsection{Flow Charts}

\begin{figure}[htbp]
	\centering
		\includegraphics[width=0.8\textwidth]{CASPDMFLOWCHARTA.pdf}
	\caption{Flow Chart 1}
	\label{fig:fcA}
\end{figure}

\begin{figure}[htbp]
	\centering
		\includegraphics[width=0.9\textwidth]{CASPDMFLOWCHARTB.pdf}
	\caption{Flow Chart 2}
	\label{fig:fcB}
\end{figure}



==> 3-Examples.tex <==
\section{Examples}

Description of the running examples which will be developed along the different CASP-DM phases...

\subsection{Estate agent} %Jose's example

From \cite{Hernandez-Orallo2015}. An estate agent has a database of possible customers who are interested in buying a house. The estate agent collects information about each customer and learns a model about the maximum mortgage that the customer can get from a bank. This is our regression model. On an everyday basis, several new properties enter the estate agents portfolio. Each of them has a different price. Obviously, the estate agent only offers a property to those customers that can afford it, i.e., those that can get a mortgage for at least the property price1. That means that each property represents a genuine cutoff of customers, those who can afford the property and those who cannot. 


\subsection{Retail group} %Nando's example
From \cite{Martinez:Orallo:ECML15}. This is an artificial dataset constructed from IBM sales information. It contains sales data for coffee and tea products sold in stores across the United States \cite{aroma_web}. The  data is almost directly converted into a multidimensional datamart where each fact describes the sales of products in dollars according  according to five dimensions (hierarchies in parenthesis):

	{\sf PROMO} ($\mbox{\sf KeyPromo} < \mbox{\sf PromoType} < \mbox{\sf All}$),
	{\sf CLASS} ($\mbox{\sf KeyClass} < \mbox{\sf All}$),
	{\sf PRODUCT} ($\mbox{\sf KeyProduct} < \mbox{\sf All}$),
	{\sf STORE} ($\mbox{\sf KeyStore} < \mbox{\sf KeyMKT} < \mbox{\sf MKT-HQ-City} < \mbox{\sf MKT-HQ-State} < \mbox{\sf MKT-District} < \mbox{\sf MKT-Region} < \mbox{\sf All}$) and
	{\sf PERIOD} ($\mbox{\sf Year}$).
	
	%Note that as we use the {\sf PERIOD} dimension to split the data we only consider one level here. 
\noindent Data goes from years 2004 to 2006 and the number of possible multidimensional contexts is $3 \times 2 \times 2 \times 7 \times 1 = 84$.

%
%\begin{itemize}
	%\item $X_1$ (product): ID\_product >  category > department
	%\item $X_2$ (location): ID\_Store > City > Region
	%\item $X_3$ (time): Day > Month > Trimester > Year
%\end{itemize}
          




\subsection{Activity Recognition in Smart Homes} %Peter's Example

From \cite{twomey2016sphere}. The  task  is   to do reliable activity recognition and prediction for  every second of the test data using the sensor data provided. Training data will be in the form of long sequences of data (tens of minutes in length), while test data will be short sequences, typically of length 10-30 seconds. Predictions must be made for every second of data. Contexts include resident identity, number of residents, house layout. 

\subsection{Washington Bike Rental} %Nicolas' example

CASE: continuous input reframing, eg. washington bike rental. Applies to relational aggregates similarly. Predict the number of available bikes. Rather customer satisfaction. 


\subsection{Basket analysis} %Nicolas' example

CASE: association rules, eg. basket analysis.

\subsection{MoReBikeS: Model Reuse with Bike Rental Station data} %Meelis' example

From \cite{kullmorebikes}. Bike rental company needs to move bikes around to avoid empty and full stations. The task is to predict the number of bikes available at a particular rental station 3 hours later, given some history data. Some stations are new and have short history of data. There is a long-term trend in time in bike usage. Information from older stations should be used to improve performance on younger ones. In detail, the overall data-set is obtained from 275 bike rental stations located in Valencia, Spain. For the participants, everyone gets access to the data for all the 275 stations during the October of 2014 and use these data as training data. 6 trained linear regression models are also provided for each station from station 1 to station 200. These linear regression models are trained with the data that covers the whole year of 2014. Therefore, the task of the challenge is, by reusing these trained models and limited training data, to predict the number of available bike at some new bike stations (station 201 to station 275).


